Post-Nonlinear Sparse Component Analysis Using Single-Source Zones and Functional Data Clustering

In this paper, we introduce a general extension of linear sparse component analysis (SCA) approaches to postnonlinear (PNL) mixtures. In particular, and contrary to the state-of-art methods, our approaches use a weak sparsity source assumption: we look for tiny temporal zones where only one source is active. We investigate two nonlinear single-source confidence measures, using the mutual information and a local linear tangent space approximation (LTSA). For this latter measure, we derive two extensions of linear single-source measures, respectively based on correlation (LTSA-correlation) and eigenvalues (LTSA-PCA). A second novelty of our approach consists of applying functional data clustering techniques to the scattered observations in the above single-source zones, thus allowing us to accurately estimate them.We first study a classical approach using a B-spline approximation, and then two approaches which locally approximate the nonlinear functions as lines. Finally, we extend our PNL methods to more general nonlinear mixtures. Combining single-source zones and functional data clustering allows us to tackle speech signals, which has never been performed by other PNL-SCA methods. We investigate the performance of our approaches with simulated PNL mixtures of real speech signals. Both the mutual information and the LTSA-correlation measures are better-suited to detecting single-source zones than the LTSA-PCA measure. We also find local-linear-approximation-based clustering approaches to be more flexible and more accurate than the B-spline one.

==> Figures/schema_block_BSSstruct.tex <==
\begin{pgfpicture}{0cm}{-0.5cm}{7.25cm}{1.5cm}
        \pgfputat{\pgfxy(0,0)}{\pgfbox[left,base]{$s_N$}}
        \pgfputat{\pgfxy(0,0.5)}{\pgfbox[left,base]{$\vdots$}}
        \pgfputat{\pgfxy(0,1)}{\pgfbox[left,base]{$s_1$}}
        \pgfsetendarrow{\pgfarrowsingle}
        \pgfline{\pgfxy(0.5,0)}{\pgfxy(1,0)}
        \pgfline{\pgfxy(0.5,1)}{\pgfxy(1,1)}
        \pgfrect[stroke]{\pgfxy(1,-.1)}{\pgfxy(1,1.2)}
        \pgfputat{\pgfxy(1.5,0.5)}{\pgfbox[center,center]{$A$}}
        \pgfsetendarrow{\pgfarrowsingle}
        \pgfline{\pgfxy(2,0)}{\pgfxy(2.75,0)}
        \pgfline{\pgfxy(2,1)}{\pgfxy(2.75,1)}
        \pgfputat{\pgfxy(2.25,.25)}{\pgfbox[center,base]{$z_P$}}
        \pgfputat{\pgfxy(2.25,1.2)}{\pgfbox[center,base]{$z_1$}}
        \pgfcircle[stroke]{\pgfxy(3,0)}{0.25cm}
        \pgfcircle[stroke]{\pgfxy(3,1)}{0.25cm}
        \pgfputat{\pgfxy(3,0)}{\pgfbox[center,center]{$f_P$}} 
        \pgfputat{\pgfxy(3,0.6)}{\pgfbox[center,center]{$\vdots$}}               
        \pgfputat{\pgfxy(3,1)}{\pgfbox[center,center]{$f_1$}}   
        \pgfsetendarrow{\pgfarrowsingle}
        \pgfline{\pgfxy(3.25,0)}{\pgfxy(4,0)}
        \pgfline{\pgfxy(3.25,1)}{\pgfxy(4,1)}
        \pgfputat{\pgfxy(3.5,.25)}{\pgfbox[center,base]{$x_P$}}
        \pgfputat{\pgfxy(3.5,1.2)}{\pgfbox[center,base]{$x_1$}}  
        \pgfcircle[stroke]{\pgfxy(4.25,0)}{0.25cm}
        \pgfcircle[stroke]{\pgfxy(4.25,1)}{0.25cm}
        \pgfputat{\pgfxy(4.25,0)}{\pgfbox[center,center]{$g_P$}}
        \pgfputat{\pgfxy(4.25,0.6)}{\pgfbox[center,center]{$\vdots$}}           
        \pgfputat{\pgfxy(4.25,1)}{\pgfbox[center,center]{$g_1$}} 
        \pgfline{\pgfxy(4.5,0)}{\pgfxy(5.25,0)}
        \pgfline{\pgfxy(4.5,1)}{\pgfxy(5.25,1)}
        \pgfputat{\pgfxy(4.75,.25)}{\pgfbox[center,base]{$e_P$}}
        \pgfputat{\pgfxy(4.75,1.2)}{\pgfbox[center,base]{$e_1$}}   
        \pgfrect[stroke]{\pgfxy(5.25,-.1)}{\pgfxy(1,1.2)}
        \pgfputat{\pgfxy(5.75,0.5)}{\pgfbox[center,center]{``$A^{-1}$''}}                           
        \pgfsetendarrow{\pgfarrowsingle}
        \pgfline{\pgfxy(6.25,0)}{\pgfxy(7,0)}
        \pgfline{\pgfxy(6.25,1)}{\pgfxy(7,1)}
        \pgfputat{\pgfxy(7.25,0)}{\pgfbox[left,base]{$y_N$}}
        \pgfputat{\pgfxy(7.25,0.5)}{\pgfbox[left,base]{$\vdots$}}        
        \pgfputat{\pgfxy(7.25,1)}{\pgfbox[left,base]{$y_1$}}
\end{pgfpicture}
